Efficient and Expressive Bytecode-Level Instrumentation for Java Programs

We present an efficient and expressive tool for the instrumentation of Java programs at the bytecode-level. BISM (Bytecode-Level Instrumentation for Software Monitoring) is a light-weight Java bytecode instrumentation tool that features an expressive high-level control-flow-aware instrumentation language. The language is inspired by the aspect-oriented programming paradigm in modularizing instrumentation into separate transformers, that encapsulate joinpoint selection and advice inlining. BISM allows capturing joinpoints ranging from bytecode instructions to methods execution and provides comprehensive static and dynamic context information. It runs in two instrumentation modes: build-time and load-time. BISM also provides a mechanism to compose transformers and automatically detect their collision in the base program. Transformers in a composition can control the visibility of their advice and other instructions from the base program. We show several example applications for BISM and demonstrate its effectiveness using three experiments: a security scenario, a financial transaction system, and a general runtime verification case. The results show that BISM instrumentation incurs low runtime and memory overheads.

==> compositionsummary.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white},
  root/.style     = {shape=circle,align=center, font=\normalsize},
  env/.style      = {shape=circle,align=center, font=\normalsize},
  leaf/.style     = {shape=circle,align=center,font=\small, outer sep=0pt},
  dummy/.style    = {circle,draw}
}
\begin{tikzpicture}
  [
    grow                    = right,
    sibling distance        = 6em,
    level distance          = 10em,
    level/.style={sibling distance = 3cm/#1,
  level distance = 4.5cm},
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
  \node [root] {Interference ?}
  child { node [env] {Order Doesn't Matter}
    edge from parent node [below] {no} }
  child { node [env] {Want Visbility ?}
    child { node [leaf] { Order Matters \\ Specify Correct Order}
      edge from parent node [below] {yes} }
    child { node [leaf] {Order Doesn't Matter\\ + Use @Hidden}
            edge from parent node [above, align=center]
              {no}
            }
    edge from parent node [above] {yes} };
\end{tikzpicture} 

==> staticanalysis.tex <==
\section{Static Analysis meets Runtime Verification}
\label{sec:staticanalysis}

In this section, we demonstrate how static analysis can be combined with runtime verification in BISM.  
%
In runtime verification, a trace of events is extracted from a running program in order to check for the violation or satisfaction of a desired property.
%
An event maps to a specific action from the monitored program (a method call, instruction, etc.), and the program is exhaustively instrumented to capture all executions of related instructions.
%

In our work, we show how static analysis can be applied to potentially detect "safe" execution paths in the control flow graph of a method that if executed at runtime they are guaranteed to preserve the monitored property.
%
For monitoring, there is no need to extract events from instructions found in such paths and the transformer performing static analysis in BISM can mark their shadows as hidden from instrumentation.
%
This results in optimizing the instrumentation of a target program.
% 
We start by introducing our running example of a Java program that creates a collection and associated iterator.
%

\begin{example}[UnSafeIterator in Java]
    \label{ex:unsafeIterator}

Listing \ref{lst:unsafeIterator}, shows an example of a Java program creating a collection, 
an iterator, and calling next operation on the iterator. 
%
Java specifies that a collection should not be updated when an iterator associated with it is being used, know as \textit{UnSafeIterator} property.  
%
We can see that if the lines 7-8 are executed at runtime, then the property is violated.
%
   
    \begin{lstlisting}[style=JavaStyle,
        backgroundcolor=\color{white}, 
        caption={Unsafe usage of iterator in Java.}, 
      captionpos=b,
      label=lst:unsafeIterator,
      float=hbtp,
      frame=bt
    ]
    List list = new ArrayList<>();
    list.add(..); 

    Iterator it = list.iterator();

    if(some_condition) {
        list.add(..); 
        list.add(..); 
    }
    
    doSomething(it.next()); 

    it = list.iterator(); 
    it.next(); 

  \end{lstlisting}
\end{example}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Monitoring a Property}
\label{sec:property}

Runtime verification is the process of checking a property on a trace (finite sequence) of events.
%
In the context of our work, an event records an action from the monitored program (a method call, instruction, etc.).
%
BISM provides an expressive language to instrument the code to extract events during a program execution and pass it to a monitor.
%
We proceed with an example that shows a BISM transformer to instrument the program from  Example \ref{ex:unsafeIterator}.



\begin{example}[UnSafeIterator Instrumentation]
\label{ex:unsafeIteratorMonitoring}
For runtime verification, to check for the \textit{UnSafeIterator} property, we need to instrument the program to extract the needed events.
%
Listing \ref{lst:unsafeIteratorTransformer}, shows a BISM transformer that captures method calls \textit{list.iterator()}, \textit{list.add()}, \textit{it.next()} with the \textit{onMethodCall} joinpoint.
%
The method \ttt{emit()} omitted for brevity, sends an event to an external monitor.
%
Captured method calls are emitted as abstracted events $Events = \{ c, u, n \}$ which represent the creation of an iterator, an update operation on the collection, and calling next on the iterator respectively.
%
The program in Example \ref{ex:unsafeIterator}, the program will be instrumented at 7 locations to emit event $c$ before lines (4,13), $u$ before lines (2,7,8), and $n$ before lines (11,14). 
%   
\begin{lstlisting}[style=JavaStyle,
    backgroundcolor=\color{white}, 
    caption={BISM transformer to capture events for \textit{UnSafeIterator} property}, 
    captionpos=b,
    label=lst:unsafeIteratorTransformer,
    numbers = none,
    float=hbtp,
    frame=bt
]
@Override
public void beforeMethodCall(MethodCall mc, MethodCallDynamicContext dc) {

    if (mc.methodName.contains("iterator") && mc.methodOwner.contains("List")) {
        emit("c");
    }
    if (mc.methodName.contains("add") && mc.methodOwner.contains("List")) {
        emit("u");
    }
    if (mc.methodName.contains("remove") && mc.methodOwner.contains("List")) {
        emit("u");
    }
    if (mc.methodName.contains("next") && mc.methodOwner.contains("Iterator")) {
        emit("n");
    }
}
  \end{lstlisting}
  \end{example}


We now discuss some preliminaries and notation about bad and good prefixes and what it means to monitoring.
%
Let $\Sigma$ be the set of events, $\Sigma^*$ the set of all finite traces over $\Sigma$, and  $\Sigma^\omega$  the set of all infinite traces over $\Sigma$.
%
We now recall the notions of good and bad prefixes from~\cite{Kupferman2001}.
%

\begin{definition}[Bad/Good prefixes~\cite{Kupferman2001}]
    Given a language $L \subseteq \Sigma^\omega$ of infinite words over $\Sigma$, we call a finite word $u \in \Sigma^*$:
    
    \begin{itemize}
        \item a \textit{bad} prefix for $L$, if $\forall w \in \Sigma^\omega$ : $u w \notin L$
        \item a \textit{good} prefix for $L$, if $\forall w \in \Sigma^\omega$: $u w \in L$
    \end{itemize}
\end{definition}

%
\begin{remark}
    \label{remark:extensionClosed}
    The language of a bad (good) prefix is extension-closed since every continuation of a bad (good) prefix for a language $L$ by a finite word is also a bad (good) prefix for $L$.
\end{remark}

We now recall the definition of safety and co-safety languages from~\cite{Kupferman2001}.
\begin{definition}[Safety and Co-Safety Languages~\cite{Kupferman2001}]
   A language $L \subseteq \Sigma^\omega$ is called
   \begin{itemize}
    \item  a safety language, if for all $w \notin L$, there exist a prefix $u \in \Sigma^*$ of $w$ which is a \textit{bad} prefix for $L$.
    \item  a co-safety language, if for all $w \in L$, there exist a prefix $u \in \Sigma^*$ of $w$ which is a \textit{good} prefix for $L$.
\end{itemize}
\end{definition}

A property $\varphi$ (defined in any suitable formalism), a language of infinite words, is a subset of $\Sigma^\omega$ such that $\lang(\varphi) = \{ w \in \Sigma^\omega \ | \ w \models \varphi \}$.
%
A property $\varphi$, is called a safety property (co-safety property), if the language of the property $\lang(\varphi)$, is a safety language (co-safety language).
%

\begin{property}[Bad/Good Prefixes are Co-Safety]
    \label{property:precosafety}
   The language of good and bad prefixes is a co-safety language. 
\end{property}
\paragraph{SKETCH}
    Let the language of bad/good prefixes be $L \in \Sigma^\omega$. 
    %
    For any word (bad/good prefix) $w \in L$, there exists a prefix $u \in \Sigma^*$ of $w$ which is a bad/good prefix for $L$. 
    %
    The prefix $u$ is either $w$ itself,
    %
    or $w$ is a continuation of a $u$ such that  $w \in u.\Sigma^*$.
    \todo{needs work}
 

When monitoring at runtime, we are interested in reporting a violation/satisfaction of a property from a trace as early as possible.
%
This means that for safety and co-safety properties, observing a \textit{bad} (alternatively \textit{good}) prefix in a trace generated by the program is sufficient 
to produce a final verdict since every continuation of the trace will produce the same result.
%
% So in summary, monitoring for violations of safety (co-safety) properties sums up to checking for finite prefixes of violating (satisfying) traces.
% %

\begin{example}[UnSafeIterator Monitoring]
    \label{ex:unsafeIteratorMonitoring}

To monitor for the violation of the \textit{UnSafeIterator} property from Example \ref{ex:unsafeIterator}, 
the monitor can be implemented to look for bad prefixes. 
%
The bad prefixes language can be defined as a regular language \{$c$ .$n^*$.$u^+$.$n$ .$\Sigma^*$\}.
%
The monitor can check for the occurrence of one single finite-prefix in \{$c$.$n^*$.$u^+$.$n$\}, as it suffices to find to one such word in the trace to conclude that the trace violates the property.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Constructing the Cfg Automata}
The Cfg, control-flow-graph,  of a method represents the behavior of a program by containing all the possible execution paths a program can take.
%
In this section, we describe how a Cfg is prepared and transformed into an automaton.
%
The constructed automata faithfully represents the Cfg and each state in the automata represents a shadow in the program (an instruction) that is responsible for emitting an event we are interested in.
% 
We start by describing how we discard irrelevant instructions that does not produce events we are interested in, then how we split the basic blocks into multiple nodes.
%
After that, we define our Cfg Automata.




\subsubsection{Preparing the Cfg}
The control flow graph of a method is a directed graph where nodes are basic blocks and edges represents jumps in the control flow.
%
Given a $CFG = \tuple{Blocks, Edges}$ for a method $m$, where $Blocks$ represent all basic blocks, and $Edges \subseteq Blocks \times Blocks $, we want to construct a modified graph $G= \tuple{B, E}$.

Let $Blocks.instr$ represent all instructions of blocks.
%
For a basic block $b \in Blocks$, $b.instr$ is the sequence of instructions in the block, and $b.entry$ is true if the basic block is the entry block of a method and $b.exit$ is true if the basic block is an exit block.
%
We are interested in actions (a method call, instruction, etc.) in the program that corresponds to events.
%
As such, we omit all irrelevant instructions from the basic blocks. 
%
Let $Events$ be the set of events we want to extract, $B.instr$ be all the instructions in basic blocks in $CFG = \tuple{Blocks, Edges}$. 
%
$$
Blocks.instr \ =  \   Blocks.instr.\map( i \rightarrow \funcparts{ \
i & \pif \  i \in \events , \\
\epsilon & \otherwise 
} ) \   
$$
We map all instructions that generate an event $e \in Events$, and erase all other instructions by replacing them with $\epsilon$.


\begin{definition}[Block Splitting]
    \label{def:splitNode}
    The function $split : Blocks \ \rightarrow Blocks$, splits a basic block into multiple blocks one per each instruction, is defined as follows: 
    $$ 
    \begin{matrix} 
     split(b) \ = \ \{ b_i \ | \ \forall i \in b.instr \} 
    \end{matrix}
    $$
\end{definition}
% \cup   \{  \ b_{\epsilon} \quad  \mathrm{if} \ b.exit \ = \ true \ \}
% 
After omitting irrelevant instructions from the basic blocks, we want to be able to map each instruction in the program to a unique node.
%
Definition \ref{def:splitNode}, defines a function that splits a block into multiple blocks (one per instruction).
%
We now show how to construct the modified graph from the original graph.

\begin{definition}[Modified Graph $G$]
    \label{def:modifiedGraph}

  Given a $CFG = \tuple{Blocks, Edges}$, we construct a modified graph  $G= \tuple{B, E}$ as follows:

\begin{align*}
    B \ = &\ \ \ \ \{ \ split(b) \ | \ \forall b \in Blocks \},\tag{1}\\
    E \ =   & \ \ \ \ \{ \ \tuple{b^\prime,b_i} \ |  \  \forall b^\prime \in Blocks , b_i \in split(b) : \tuple{b^\prime,b} \in Edges \\
              &  \quad \quad  \quad \quad \quad \quad \&\&  \ \ \mathrm{idx}^b_i \ = \ 0 \ \} \tag{2}\\
              & \cup  \{ \ \tuple{b_i,b_{j}}  \ |  \ \forall b_i,b_j \in split(b)  \ \ \&\& \ \ 0 \leq \mathrm{idx}^b_i  <  |b.instr| - 1 \\
              &  \quad \quad  \quad \quad \quad \quad \&\&  \ \ \mathrm{idx}^b_j  =  \mathrm{idx}^b_i + 1 \ \} \tag{3}\\
              & \cup \{ \ \tuple{b_i,b^\prime}  \ |  \  \forall b^\prime \in Blocks ,  b_i \in split(b) : \tuple{b,b^\prime} \in Edges\\
              &  \quad \quad  \quad \quad \quad \quad \&\&  \ \ \mathrm{idx}^b_i =  |b.instr| - 1 \ \} \tag{4}
\end{align*}     
   $ \quad \quad$ where $ \mathrm{idx}^b_i: b.instr \rightarrow  \mathbb{N}$ returns the index of an instruction $i$ in a block $b$.
\end{definition}

The newly created graph $G$ from Definition\ref{def:modifiedGraph}, is constructed such that: (line 1) all basic blocks in the original Cfg are split into multiple nodes, one node per instruction.
All incoming edges to an original block, are connected to the node representing the first instruction of the original block (line 2). All nodes that are created from a single original block are connected 
sequentially (line 3). All outgoing edges from the original block are now outgoing from the last split node (line 4).

\begin{remark}
    Each node in the new graph $G$ will contain one instruction, such that $\forall b \in B : |b.instr| =  1$, which is: either an instruction we are interested in that maps to an event in $Events$, or $\epsilon$. 
    %
    The entry block in the new graph, is the first split node of the original entry block $b_i \in split(b) : b \in Blocks \ \&\& \ \ b.entry = true \ \&\&   \ \mathrm{idx}^b_i \ = \ 0 $.
    %
    In implementation, we merge two consecutive nodes containing $\epsilon$, and accordingly move their edges.
\end{remark}




\subsubsection{Cfg Automaton}
We now show how the Cfg automaton is constructed from the prepared graph.

\begin{definition}[Cfg Automaton]
    \label{def:cfgAutomata}
    Given a graph $G = \tuple{B, E}$. 
    %
    The Cfg Automata is a finite state machine $\automata^c = \{\Sigma, Q, \delta, Q_0, F  \}$  constructed as follows:
  \[
    \automata^c = \\ 
    \funcparts{
        \Sigma &=   Events ,\\
         Q \ &=  \{ q_b \ | \ \forall b \in B \}, \\
         q_0 &=   \{ q_b \ | \ b \in B  \ \&\& \ b.entry = true \ \}, \\
         \delta  &=  \{ \tuple{q_b , s ,q_{b^\prime}} \ | \ \tuple{b,b^\prime} \in E \  \&\& \  b.\binstr = s  \}\\
         F &=   Q
    }
\]
\end{definition}
From Definition \ref{def:cfgAutomata}, each node in the modified control flow graph is represented in a state in the automata.
%
Moreover, since a node is representing a single instruction and the one instruction inside each node, is labelling the transitions outgoing from its state. 
%
Also, note that all states are accepting states.

\begin{property}[A Cfg Automata state corresponds to an instruction shadow]

In Section\ref{sec:shadows}, we defined the shadows of a program. Shadows represent regions in the program that BISM mark for instrumentation, a shadow can be an instruction along with the specified direction (\textit{before} and \textit{after}). 
%
From our constructed automaton, a state corresponds to an instruction $i$ in the original program and
%
by labelling the transitions outgoing from a state with the instruction $i$, we have the state representing the shadow $\tuple{\mathrm{before},i}$.
\end{property}
%

\begin{example}[Cfg Automaton]
    \label{ex:unsafeIteratorCfg}
    Figure \ref{fig:cfgAuto}, shows the Cfg automata constructed from the Java program from Example \ref{ex:unsafeIterator}.
    %
    Each state in the Cfg Automata correspond to an instruction we are interested in the program.
    %
    State 0 to line 2, state 1 to line 4, state 2 and 3 to lines 7 and 8, state 4 to line 11, state 5 to line 13, state 6 to line 14.

    \begin{figure}[t!]
        \centering
            \includegraphics[width=0.8\textwidth]{figures/cfg.png} 
            \caption{Cfg Automaton $\automata^c$} 
            \label{fig:cfgAuto}
    \end{figure}  

\end{example}    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Cutting Behaviors}
\subsubsection{Property-Violating Execution Paths}

Using the constructed Cfg automaton, we proceed to find execution paths in the program that if executed at runtime are guaranteed to violate a given property.
%
We do this by checking if the language of the Cfg automaton intersects with the language of a property $\varphi$.
%
Recall from Section \ref{sec:property}, that the language of bad prefixes is a co-safety property.
%
Given a regular co-safety property $\varphi$ over $\Sigma$, whose language is $\lang(bad_\varphi).\Sigma^*$,
%
we construct the automaton of violating words $\automata^{bad_\varphi}$.
 %

\begin{example}[Bad prefixes for UnSafeIterator property]
    \label{ex:violatingWords}

   Recall the \textit{UnSafeIterator} property that specifies that a collection should not be updated when an iterator associated with it is being used, know as \textit{UnSafeIterator} property.  
%
    The language of violating words, $\lang(bad_\varphi)$ is the regular language \{$c$.$n^*$.$u^+$.$n$\}.
%
    Figure \ref{fig:violatingAuto}, shows the automata  $\automata^{bad_\varphi}$.

    \begin{figure}[t!]
        \centering
            \includegraphics[width=0.45\textwidth]{figures/violating-pattern.png} 
            \caption{Automata that accepts $\lang(bad_\varphi)$ } 
            \label{fig:violatingAuto}
    \end{figure}
\end{example}  
 

% Recall that given a finite state machine $\automata = \{\Sigma, Q, \delta, Q_0, F  \}$, a state $q \in Q$ is reachable if there exists
% a word $s \in \Sigma^*$ such that $\delta(q_0,s)  = q$.
 
Given a Cfg Automaton $\automata^{c} = \{\Sigma, Q, \delta, Q_0, F  \}$ and an automaton for violating word $\automata^{bad_\varphi}$:
\[
    \forall q \in Q: \lang(\automata^{c}(q)) \cap  \lang(\automata^{bad_\varphi}) \neq \emptyset \\
    \implies  \textnormal{there is violating path starting from state q}
\]

This allows us to find states that are located at the beginning of execution paths that if executed will violate the property $\varphi$.
%
We now give the algorithm that marks the states in violating execution paths in the Cfg automaton. 
%
Recall that given a finite state machine $\automata = \{\Sigma, Q, \delta, Q_0, F  \}$, a state $q \in Q$ is coreachable if there exists
a word $s \in \Sigma^*$ such that $\delta(q,s)  \in F$.

\begin{algorithm}
    \label{alg:markingViolating}
    \SetAlgoLined
    \DontPrintSemicolon
    \SetKwFunction{algo}{algo}\SetKwFunction{proc}{DFS}
    let $\violating$ = \{ \}\; 
    $Q$ be the set of states in cfg automaton $\automata^{c}$\; 
    \BlankLine
    \ForEach{$q$ in $Q$}{
      $\hat \automata$ = $\automata^{c}(q) \cap  \automata^{bad_\varphi}$ \;
      \uIf{ $\hat \automata$ $\neq$ $\emptyset$}{      
            \ForEach{$q^{\prime}$ in co-reachable($\hat \automata$)}{
                $\violating$ = $\violating$ $\cup$ corresponding state of $q^{\prime}$ in $\automata^{c}$
            }
        }      
    } 
     \caption{Marking Property-violating states $\safe$}
    \end{algorithm}

 Algorithm \ref{alg:markingViolating}, shows how to mark all states in the Cfg automaton $\automata_{cfg}$  that are in a property violating path.
 %
 For each state $q$ in $\automata^{c}$ (line 3), we set $q$ as the initial and calculate the intersection with the $\automata^{bad_\varphi}$ line (4), if the intersection is not empty (line 5),
 we find the set of all co-reachable states in the intersection automata (line 6). Each state in the intersection automata  $\hat \automata$ corresponds to a state in $\automata^{c}$ and $\automata^{bad_\varphi}$.
 For each coreachable state in $\hat \automata$, we add its corresponding state in $\automata^{c}$ to the set $\violating$.
 %
 \paragraph{Diagnosis} 
 For monitoring, we have to instrument the corresponding instructions of the marked states located in the property violating paths.
 %
 Since if the program enters such path, the property will be violated.
 %
 As for the other states, their corresponding instructions will be hidden from instrumentation.
 %
 This reduces the number of instructions that needs to be instrumented in the target program.



\begin{example}[Property violating states]
    \label{ex:unsafeIteratorCfgSafe}

    Figure \ref{fig:cfgAutoSafe}, shows the Cfg automata constructed from the Java program from Example \ref{ex:unsafeIterator}, where states marked in red exist in a property violating execution path.
    %
    The red states in the automata are the states that we need to extract traces from, and the white states are hidden from instrumentation.
    %
    We can see that instead of instrumenting at 7 different locations (see Example\ref{ex:unsafeIteratorMonitoring}), we only have to instrument at 4 locations.

    \begin{figure}[t!]
        \centering
            \includegraphics[width=0.8\textwidth]{figures/cfg-violating.png} 
            \caption{Marking property violating paths } 
            \label{fig:cfgAutoSafe}
    \end{figure}
\end{example}  





\subsection{Conclusion}
